Near-optimal Algorithms for Explainable k-Medians and k-Means

We consider the problem of explainable $k$-medians and $k$-means introduced by Dasgupta, Frost, Moshkovitz, and Rashtchian~(ICML 2020). In this problem, our goal is to find a threshold decision tree that partitions data into $k$ clusters and minimizes the $k$-medians or $k$-means objective. The obtained clustering is easy to interpret because every decision node of a threshold tree splits data based on a single feature into two groups. We propose a new algorithm for this problem which is $\tilde O(\log k)$ competitive with $k$-medians with $\ell_1$ norm and $\tilde O(k)$ competitive with $k$-means. This is an improvement over the previous guarantees of $O(k)$ and $O(k^2)$ by Dasgupta et al (2020). We also provide a new algorithm which is $O(\log^{3/2} k)$ competitive for $k$-medians with $\ell_2$ norm. Our first algorithm is near-optimal: Dasgupta et al (2020) showed a lower bound of $\Omega(\log k)$ for $k$-medians; in this work, we prove a lower bound of $\tilde\Omega(k)$ for $k$-means. We also provide a lower bound of $\Omega(\log k)$ for $k$-medians with $\ell_2$ norm.

==> paper/terminal-embedding.tex <==
\section{Terminal Embedding}\label{sec:terminal_embedding}

\begin{lemma}\label{lem:terminal-1d}
For every finite set of real numbers $K$, the function $\psi_K$ defined in Lemma~\ref{lem:embedding} is a cut preserving embedding that satisfies for every $x\in \bbR$ and $y\in K$
\begin{align*}
|\psi_K(x)- \psi_K(y)|&\leq
|x-y|^2\\
& \leq 8|K|\cdot|\psi_K(x)- \psi_K(y)|. 
\end{align*}
\end{lemma}

\begin{proof}
We first show that this function $\psi_K$ is continuous and differentiable in $\bbR$. Consider $2k$ open intervals on the real line divided by points in $K$ and points $(y_i+y_{i+1})/2$ for $i\in \{1,2,\cdots,k-1\}$. In every such open interval, the function $\psi_K$ is a quadratic function, which is continuous and differentiable. Since $\psi_K$ is also continuous and differentiable at the endpoints of these intervals, the function $\psi_K$ is continuous and differentiable in $\real$. For any $x \in \bbR$, we have $\psi_K'(x) = 2\abs{x-y^*} \geq 0$ where $y^*$ is the closest point in $K$ to $x$. Thus, the function $\psi_K$ is increasing in $\bbR$, which implies $\psi_K$ is cut preserving.  

We now prove that $\psi_K$ satisfies two inequalities. We first show that for every $x\in \bbR$ and $y \in K$, 
$|\psi_K(x)-\psi_K(y)|\leq 
|x-y|^2$. Suppose that $x\geq y$ (The case $x\leq y$ is handled similarly.) If $x=y$, then this inequality clearly holds. Thus, to prove $|\psi_K(x)-\psi_K(y)|\leq |x-y|^2$, it is 
sufficient to prove the following inequality on derivatives 
$$(\psi_K(x)-\psi_K(y))'_x\leq \big((x-y)^2\big)'_x.$$
Let $y^*$ be the closest point in $K$ to $x$. Then,
\begin{multline*}
(\psi_K(x)-\psi_K(y))'_x = (\psi_K(x))'_x = \\
= (\psi_K(y^*) + \varepsilon_x(x-y^*)^2)'_x 
= 2|x-y^*|.
\end{multline*}
Since $y^*$ is the closest point in $K$ to $x$, we have 
$|x-y^*|\leq |x-y| = \big((x-y)^2\big)'_x /2$.
This finishes the proof of the first inequality.

\medskip

We now verify the second inequality. First, consider 
two points $y_i$ and $y_j$ ($y_i < y_j$). Write,
$$\psi_K(y_j) - \psi_K(y_i) = z_j - z_i =
\frac{1}{2} \sum_{m=i}^{j-1} (y_{m+1}-y_m)^2.$$
By the arithmetic mean--quadratic mean inequality, we have
$$
(j-i)\cdot \sum_{m=i}^{j-1} (y_{m+1}-y_m)^2 \geq
\Big(\sum_{m=i}^{j-1} y_{m+1}-y_m\Big)^2 = 
(y_j - y_i)^2.
$$
Thus,
$$\psi_K(y_j) - \psi_K(y_i)\geq \frac{(y_j-y_i)^2}{2(j-i)}\geq 
\frac{(y_j-y_i)^2}{2(k-1)}.$$

Now we consider the case when $x$ is an arbitrary real number in $\bbR$ and $y\in K$. Let $y^*$ be the closest point in $K$ to $x$. Then,
$$|x-y|^2 \leq 2|x-y^*|^2 + 2|y^*-y|^2.$$
The first term on the right hand side equals
$4|\psi_K(x)-\psi_K(y^*)|$; the second term is upper bounded by $4(k-1) |\psi_K(y)-\psi_K(y^*)|$. Thus,
$$|x-y|^2 \leq 4|\psi_K(x)-\psi_K(y^*)| +
4(k-1) |\psi_K(y^*)-\psi_K(y)|.$$
Note that $|\psi_K(x)-\psi_K(y^*)|\leq |\psi_K(x)-\psi_K(y)|$ since $y^*$ is the closest point in $K$ to $x$. Also, we have
\begin{align*}
|\psi_K(y^*)&-\psi_K(y)|\leq \\
&\leq |\psi_K(x)-\psi_K(y^*)| + |\psi_K(x)-\psi_K(y)|\\
&\leq 2|\psi_K(x)-\psi_K(y)|.
\end{align*}
Hence,
$$|x-y|^2 \leq 8k|\psi_K(x)-\psi_K(y)|.$$
This completes the proof.
\end{proof}

\begin{lemma}\label{lem:terminal-cut-preserving}
The terminal embedding $\psi$ is coordinate cut preserving. For every threshold cut $(i,\theta)$, there exists
a threshold cut $(i,\theta')$ such that 
$$
\{x\in \bbR^d: x_i \leq \theta'\} = \{x\in \bbR^d: \psi(x)_i \leq \theta\}.
$$
\end{lemma} 

\begin{proof}
By the construction of $\varphi$, we have for any threshold cut $(i,\theta)$
$$
\{x\in \bbR^d: \psi(x)_i \leq \theta\} = \{x\in \bbR^d: \psi_i(x_i) \leq \theta\}.
$$
Since $\psi_{i}$ is a cut preserving terminal embedding by Lemma~\ref{lem:terminal-embedding-1d}, there exists a threshold $\theta' \in \bbR$ such that
$$
\{x\in \bbR^d: x_i \leq \theta'\} = \{x\in \bbR^d: \psi_{i}(x_i) \leq \theta\}.
$$
\end{proof}
